Non-Blocking Doubly-Linked Lists with Good Amortized Complexity

We present a new non-blocking doubly-linked list implementation for an asynchronous shared-memory system. It is the first such implementation for which an upper bound on amortized time complexity has been proved. In our implementation, operations access the list via cursors. Each cursor is associated with an item in the list and is local to a process. The implementation supports two update operations, insertBefore and delete, and two move operations, moveRight and moveLeft. An insertBefore(c, x) operation inserts an item x into the list immediately before the cursor c's location. A delete(c) operation removes the item at the cursor c's location and sets the cursor to the next item in the list. The move operations move the cursor one position to the right or left. The update operations use single-word Compare&Swap instructions. The move operations only read shared memory and never change the state of the data structure. If all update operations modify different parts of the list, they run completely concurrently. Let cp(op) be the maximum number of active cursors at any one time during the operation op. The amortized complexity of each update operation op is O(cp(op)) and each move operation is O(1). We have written a detailed correctness proof and amortized analysis of our implementation.

==> cursor.tex <==
\paragraph{Cursors}
%The pseudo-code for our implementation is given in Figure \ref{code1} and \ref{code2}.
A process calls createCursor to create a new cursor $c$ and sets its $node$ to the first node in the list.
All other operations are called with cursors.
If resetCursor($c$) is called, it sets $c.node$ to the first node in the list.


%To avoid the ABA problem, when the $nxt$ or $prv$ field of a node is changed from a node $old$ to other node, $x$ is removed from the list.
%So, sometimes, $x$ would be replaced with a new copy. 
At the beginning of an update or a move operation that is called with a cursor $c$, {\bf updateCursor} is called.
If the node of $c$ is changed for the last time by another process, the updateCursor sets $c.node$ to the node that $c$ is associated with (according to the sequential specification).
First, updateCursor reads $c.node$.
If $c.node$ is removed from the list, $c.node$ must move to the next node in the list at the time of deletion, and if $c.node$ is replaced with a new copy, $c.node$ must set to the new copy.
%If $c.node$ is removed or replaced by an operation called by $p$, $c.node$ is set to the next node in the list or the new copy before the operation terminates.
%Otherwise, if the next operation called with $c$ is not resetCursor, $c.node$ will be updated at the beginning of the operation.
Before a node is replaced by a new copy, the $state$ of the node is set to copied and the $copy$ pointer of the node is set to the new copy. 
Before a node is removed from the list, the $state$ of the node is set to marked, and after removal, no operation changes the $nxt$ and $prv$ fields of the node.
So, the $nxt$ field of the removed node always points to the next node in the list at the time of removal.
%We say a node is {\it reachable} if there is path of $nxt$ pointer from $head$ to the node.

%Now, we describe how $c.node$ is updated inside updateCursor.
%If $c.node$ is changed by operations called by processes other than $p$, we describe how $c.node$ is updated inside the updateCursor routine. 
To update $c.node$, first the operation reads its $state$.
If the $state$ of $c.node$ is not ordinary and it is not reachable (line \ref{updateCursor-check}), then $c.node$ is either removed from the list or replaced with a new copy.
So, $c.node$ would be set to $node.copy$ (line \ref{updateCursor-set-new-copy}) or $node.nxt$ (line \ref{updateCursor-set-nxt}) depending on the value of its $state$. 
Then, the process reads the $state$ of the updated node and checks whether it is reachable.
If the node is not reachable, the process repeats the updating steps until it reaches a reachable node.

If $c.node$ is invalidated by an insertBefore operation, createCursor($c$) sets $invIns$ to true (line \ref{updateCursor-set-invalidIns}) and 
if $c.node$ is invalidated by a delete operation, createCursor($c$) sets $inv$ to true (line \ref{updateCursor-set-invalid}).
At the end, the updateCursor returns the value of $c.node$, its $info$, its $nxt$ and $prv$ pointer and the value of $inv$ and $invIns$ (line \ref{updateCursor-return}).


